The T05 System for The VoiceMOS Challenge 2024: Transfer Learning from Deep Image Classifier to Naturalness MOS Prediction of High-Quality Synthetic Speech

We present our system (denoted as T05) for the VoiceMOS Challenge (VMC) 2024. Our system was designed for the VMC 2024 Track 1, which focused on the accurate prediction of naturalness mean opinion score (MOS) for high-quality synthetic speech. In addition to a pretrained self-supervised learning (SSL)-based speech feature extractor, our system incorporates a pretrained image feature extractor to capture the difference of synthetic speech observed in speech spectrograms. We first separately train two MOS predictors that use either of an SSL-based or spectrogram-based feature. Then, we fine-tune the two predictors for better MOS prediction using the fusion of two extracted features. In the VMC 2024 Track 1, our T05 system achieved first place in 7 out of 16 evaluation metrics and second place in the remaining 9 metrics, with a significant difference compared to those ranked third and below. We also report the results of our ablation study to investigate essential factors of our system.

==> section/05.tex <==
\Section{Results}
\label{sec:results}


\Subsection{Effectiveness of Fusing Spectrogram Features and SSL Features}
\label{sec:fusion-result}


For correlation-based metrics, we can see from \Table{comparison_of_models} that all of our three models--namely the spectrogram-only model, the SSL-only model, and their fusion model--outperformed both baseline models in all metrics. Furthermore, in correlation-based metrics, while there is little difference in scores between the spectrogram-only model and the SSL-only model, the fusion model shows a significant improvement in scores compared to these two models. These results indicate that our systems are more effective for zoomed-in MOS prediction compared to the existing baseline systems, particularly in correlation-based metrics, and also suggest the effectiveness of fusing spectrogram and SSL features in these metrics.

For MSE, it can be seen that the spectrogram-only model achieved the best score, whereas the SSL-only model did not perform as well. Also, for MSE, although the fusion model performed better than the SSL-only model, it did not outperform the spectrogram-only model.

In comparison with the human-annotated MOS, our fusion system showed better scores than ``BVCC MOS'' in all metrics except for system-level MSE. Additionally, for system-level correlation-based metrics, our system outperformed ``sarulab-data''. 


\Subsection{Effectiveness of 2 step learning}
\label{sec:2step-result}

\input{table/comparison_of_2_step_learning}



\Subsection{Results of ablation Study on Datasets}
\label{sec:ablation_study_result}

\input{table/ablation_study.tex}


% \Subsection{Voice MOS Challenge 2024 Results}

% In the track1, both utterlance-level (Utt.) and system-level (Sys.) metrics are calculated for 25\% and 12\% heighest-rated systems, respectively. The official evaluation results are shown in \Table{official_results}. Our T05 system achieved first place in 7 out of 16 metrics and ranked second in the remaining 9 metrics, thereby securing either first or second place in all metrics. Additionally, it is notable that there is a significant difference compared to those ranked third and below.

%\input{table/official_results.tex}

==> table/official_results.tex <==
\begin{table*}[tb]
    \centering
    \setlength{\tabcolsep}{1mm} 
    \caption{Official evaluation results of the VMC2024 Track1. \textbf{Bold} and \underline{italic} scores ranked the first and second, respectively. Our system ``T05'' achieves the best 7 out of 16 metrics and ranked
second in the remaining 9 metrics. ``B01'' is the baseline system for this track.}
    \label{tbl:official_results}
    \scalebox{0.9}{
        \begin{tabular}{l|cccccccccccccccc}
            \toprule
                                 &      \multicolumn{8}{c}{Zoom-in rate: 25\%}     & \multicolumn{8}{|c}{Zoom-in rate: 12\%} \\
                                 &              \multicolumn{4}{c}{Utterance-level}                      &              \multicolumn{4}{|c}{System-level}                        &              \multicolumn{4}{|c}{Utterance-level}                     &              \multicolumn{4}{|c}{System-level}                        \\
                                 &             MSE\zj &             LCC\zk &            SRCC\zk &            KTAU\zk &           \tbhline{MSE\zj}&             LCC\zk &            SRCC\zk &            KTAU\zk &           \tbhline{MSE\zj}&             LCC\zk &            SRCC\zk &            KTAU\zk &           \tbhline{MSE\zj}&             LCC\zk &            SRCC\zk &            KTAU\zk \\
            \midrule
            B01              &              1.154 &              0.508 &              0.509 &              0.358 &            \tbhline{0.998}&              0.750 &              0.745 &              0.539 &            \tbhline{0.741}&              0.422 &              0.417 &              0.285 &            \tbhline{0.589}&              0.608 &              0.609 &              0.444 \\
            \midrule
            T01              &              0.358 &             0.490 &               0.491 &              0.342 &            \tbhline{0.162}&              0.703 & 
                  0.700 &              0.495 &            \tbhline{0.296}&              0.402 &              0.421 &              0.286 &            \tbhline{0.127}& 
                    0.540 &              0.513 &              0.333 \\
            T02              &              0.355 &             0.550 &               0.555 &              0.394 &            \tbhline{0.141}&              0.789 & 
                  0.769 &              0.578 &            \tbhline{0.410}&              0.520 &              0.544 &              0.377 &            \tbhline{0.240}& 
                    0.745 &              0.702 &              0.467 \\
            T03              &              0.406 &             0.471 &               0.488 &              0.344 &            \tbhline{0.200}&              0.674 & 
                  0.672 &              0.483 &            \tbhline{0.264}&              0.481 &              0.514 &              0.357 &            \tbhline{0.082}& 
                    0.779 &              0.768 &              0.539 \\
            T04              &              0.718 &             0.421 &               0.391 &              0.272 &            \tbhline{0.494}&              0.728 & 
                  0.698 &              0.512 &            \tbhline{0.457}&              0.311 &              0.281 &              0.191 &            \tbhline{0.270}& 
                    0.571 &              0.549 &              0.364 \\
            T05              &              \underline{0.287} &             \textbf{0.686} &               \textbf{0.679} &              \textbf{0.497} &            \tbhline{\underline{0.073}}&              \textbf{0.944} & 
                  \underline{0.940} &              \underline{0.773} &            \tbhline{\textbf{0.203}}&              \textbf{0.654} &              \underline{0.658} &              \underline{0.464} &            \tbhline{\textbf{0.056}}& 
                    \underline{0.834} &              \underline{0.788} &              \underline{0.610} \\
            T06              &              \textbf{0.255} &             \underline{0.658} &               \underline{0.676} &              \underline{0.493} &            \tbhline{\textbf{0.047}}&              \underline{0.931} & 
                  \textbf{0.943} &              \textbf{0.793} &            \tbhline{\underline{0.221}}&              \underline{0.629} &              \textbf{0.695} &              \textbf{0.505} &            \tbhline{\underline{0.057}}& 
                    \textbf{0.890} &              \textbf{0.952} &              \textbf{0.824} \\
            T07              &             0.753 &              0.377 &               0.359 &              0.254 &            \tbhline{0.446}&              0.724 & 
                  0.675 &              0.493 &            \tbhline{0.517}&              0.300&               0.294 &              0.207 &            \tbhline{0.251}& 
                    0.676 &              0.672 &              0.444 \\
%            Zoomed-in data       &              0.416 &              0.631 &              0.615 &              0.454 &            \tbhline{0.116}&              0.897 &              0.903 &              0.729 &            \tbhline{0.347}&              0.603 &              0.589 &              0.432 &            \tbhline{0.109}&              0.804 &              0.788 &              0.602 \\
            \bottomrule
        \end{tabular}
    }
\end{table*}




==> zoomed-in.tex <==
🔍

